Variable Selection for Comparing High-dimensional Time-Series Data

Given a pair of multivariate time-series data of the same length and dimensions, an approach is proposed to select variables and time intervals where the two series are significantly different. In applications where one time series is an output from a computationally expensive simulator, the approach may be used for validating the simulator against real data, for comparing the outputs of two simulators, and for validating a machine learning-based emulator against the simulator. With the proposed approach, the entire time interval is split into multiple subintervals, and on each subinterval, the two sample sets are compared to select variables that distinguish their distributions and a two-sample test is performed. The validity and limitations of the proposed approach are investigated in synthetic data experiments. Its usefulness is demonstrated in an application with a particle-based fluid simulator, where a deep neural network model is compared against the simulator, and in an application with a microscopic traffic simulator, where the effects of changing the simulator's parameters on traffic flows are analysed.

==> backup/proposal-backup-June-07-2024.tex <==





\begin{figure}
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.5]{figures/section-proposal/illustration-idea.png}
    \caption{Illustration of the proposed method "Time Slicing Variable Selection".}
    \label{fig:example-time-slicing-iid-idea-a}
  \end{subfigure}%
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/section-proposal/iid-time-bucket.png}
    \caption{Illustration of the slicing operation.}
    \label{fig:example-time-slicing-iid-idea-b}
  \end{subfigure}
  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[scale=0.4]{figures/section-proposal/illustration-bucket-and-interval.png}
    \caption{Dividing time steps into buckets and intervals $\IntervalIndex{\bucket}$.}
    \label{fig:example-time-slicing-iid-idea-c}
  \end{subfigure}

  \caption{
      (a): An intuitive illustration of the proposed method "Time Slicing Variable Selection".
      Two time series $X, Y$ have $\TimeN=130$ time steps.
      A time step at $t$ consists of a $D=5$ dimensional vector.
      The proposed method segments $\TimeN$ time steps into a set of buckets $\{\bucketIndex{1}, ..., \bucketIndex{3} \}$.
      A bucket $\bucketIndex{1}$ consists of an interval $\IntervalIndex{1}$ that is the wine-red coloured rectangle.
      A variable selection task is executed in each bucket and variables $S$ are selected, which is blue highlighted. 
      Section~\ref{sec:proposed-method} has a detailed description.
      (b): An example of the slicing operation.
      The plot at the top is the original time series.
      The slicing operation splits the original time series, randomly ordering the sequence.
      (c): Example of dividing a time-series having $T=130$ into three buckets and splitting the $\IntervalIndex{1}$ into $\IntervalIndexTrain{1}$ and $\IntervalIndexTest{1}$.
      $T=130$ and 3 buckets are the same settings as "Example" in Section~\ref{sec:example-time-slicing-variable-selection}.
  }
  \label{fig:example-time-slicing-iid}
  
\end{figure}



\subsection{Variable Selection for Two Sample Testing}
\label{sec:variable-selection-for-two-sample-testing}

Variable selection for two sample testing is a task, given $\datasetX = \{x_1, ...., x_n\}, \datasetY = \{y_1, ...., y_m\}, x_n, y_m \in \mathbb{R}^D$ sampled in i.i.d manner from two probability distributions $P, Q$, to discover a subset of variables $S \subset \{1, 2, ..., D\}$ that are responsible for discrepancies between $P, Q$ when $P \neq Q$.
The null-hypothesis $H_0 : P=Q$ and the alternative hypothesis $H_1 : P \neq Q$.
The selected variable subset $S$ is not necessarily always rejecting the $H_0$.
When the $H_0$ is truth, it is plausible that two sample testing using the selected subset $S$ accepts the $H_0$.




 
\subsection{Time-Slicing Variable Selection}
\label{sec:time-slicing-variable-selection}


The proposal is named "Time-Slicing Variable Selection".
As the name of "slicing" implies, the proposed method splits a set of time steps into a set of buckets, which we call \emph{Time Bucket}.
Figure~\ref{fig:example-time-slicing-iid-idea-a} intuitively illustrates this idea.
Suppose that two time-series $X, Y \in \mathbb{R}^{\Dim \times \TimeN}$ consisted of $\TimeN \in \mathbb{N}$ steps, and a time step $t$ consists of $\Dim$ dimensional vectors.
The proposed method divides $\TimeN$ time steps into $\TotalBucketSize \in \mathbb{N}$ buckets as shown with the wine-red coloured rectangles in Figure~\ref{fig:example-time-slicing-iid-idea-a}.
We denote $\bucketIndex{i}$ for specifying $i$-th bucket, for instance, $\bucketIndex{1}, \threeDots, \bucketIndex{3}$ in Figure~\ref{fig:example-time-slicing-iid-idea-a}.
The variable selection task is executed in each bucket $\bucket \in \{1,\threeDots,\TotalBucketSize\}$ and obtains variables $\VariableSelectionHat$, for example, two variables are selected in $\bucketIndex{1}$ at the blue highlights in Figure~\ref{fig:example-time-slicing-iid-idea-a}.

The slicing operation is exemplified in Figure~\ref{fig:example-time-slicing-iid-idea-b}.
A given time series is on the top, and the slicing operation treats all time steps as independent samples.
We put an assumption that each time step can approximate independent data points sampled from a probability distribution if the span of observation time steps is extremely small.
An example case is that a sensor observes and counts objects such as cars or particles in a quite short time spans.
In this case, the observed values do not alter dramatically in quite a small time span and thus may approximate independent samples.
Without a doubt, this assumption raises drawbacks and limitations in handling time-series data as independent samples.
We discuss these drawbacks and limitations in Section~\ref{sec:proposed-method-limitation}.

We define the time-slicing variable selection in Algorithm~\ref{alg:time-slicing-variable-selection}.
Two time-series $X, Y$ consist of $\TimeN$ time steps, $X = (x_1,...,x_\TimeN), Y = (y_1,...,y_\TimeN), X, Y \in \mathbb{R}^{\Dim \times \TimeN}$.
These two time series are generated from random processes $P, Q$ respectively.
At a time step $t$, the $D$ dimensional vector records observation values, ex. a count of simulation agents.

The proposed method iterates the variable selection and permutation test over each time bucket $\bucket$.
The algorithm table~\ref{alg:time-slicing-variable-selection} describes the procedure.
A set of time steps is $\{t_{1}, ..., t_{\TotalBucketSize}\}, 0 < t < \TimeN$, and $t_{\bucket}$ represents an end time step of a bucket $\bucket$.
In this work, we equally split $\TimeN$ time steps into $\TotalBucketSize$ buckets.
However, one can set any $t$ when one is interested in studying a specific time range.
For example, $t$ may be set to a specific step where a signal trend changes detected by a change-point detection algorithm~\citep{sin-2012}.
Corresponding to the ending time steps, we define an interval for bucket $\bucket$ as $\IntervalIndex{\bucket} = (t_{\bucket-1}, t_{\bucket}] = \{t_{\bucket-1}, \threeDots, t_{\bucket} \}$.
The algorithm requires $\ratioTrain, 0 < \ratioTrain < 1.0$ that defines a ratio of splitting the interval $\IntervalIndex{\bucket}$ into a train set $\IntervalIndexTrain{\bucket}$ and a test set $\IntervalIndexTest{\bucket}$.
Figure~\ref{fig:example-time-slicing-iid-idea-c} illustrates this operation of dividing a time series into buckets and puts a training set $\IntervalIndexTrain{\bucket}$ and a test set $\IntervalIndexTest{\bucket}$.
The function $\funcVariableSelection{\sampleSetTrain{\datasetX}_{\bucket}}{\sampleSetTrain{\datasetY}_{\bucket}}$ is a variable selection function, which we introduce in Section~\ref{sec:proposal-variable-selection}, that returns variables $\VariableSelectionHatIndex{\bucket}$.
The other two arguments of this variable selection function are $\sampleSetTrain{\datasetX}_{\bucket} = \{x_i | i \in \IntervalIndexTrain{\bucket} \}, \sampleSetTrain{\datasetY}_{\bucket} = \{y_i | i \in \IntervalIndexTrain{\bucket} \}$.
Note that $\datasetX, \datasetY$ are sets of independent samples that do not keep the temporal structure, whereas $X, Y$ are time-series.

The algorithm iterates the variable selection and permutation test over each bucket $\bucket = 1,\threeDots,\TotalBucketSize$.
At the line \ref{lst:line:define-train-test}, following the $\ratioTrain$, the algorithm randomly splits the interval $\IntervalIndex{b}$ into the train set $\IntervalIndexTrain{\IntervalIndex{\bucket}}$ and a test set $\IntervalIndexTest{\IntervalIndex{\bucket}}$.
The first is used for the variable selection task and the second is for the permutation test.
The algorithm constructs two pairs of datasets $\sampleSetTrain{\datasetX}_{\bucket} = \{x_i | i \in \IntervalIndexTrain{\bucket} \}, \sampleSetTrain{\datasetY}_{\bucket} = \{y_i | i \in \IntervalIndexTrain{\bucket} \}$ and $\sampleSetTest{\datasetX}_{\bucket} = \{x_i | i \in \IntervalIndexTest{\bucket} \}, \sampleSetTest{\datasetY}_{\bucket} = \{y_i | i \in \IntervalIndexTest{\bucket} \}$ at the line \ref{lst:line:set-X-Y}.
The variable selection task is executed with a pair of train sets $\sampleSetTrain{\datasetX}_{\bucket}, \sampleSetTrain{\datasetY}_{\bucket}$ at the line \ref{lst:line:variable-selection}.
The variable selection task obtains a set of variables $\VariableSelectionHatIndex{\bucket}$ that are responsible variables for rejecting $H_0$.
A permutation test with $\sampleSetTest{\datasetX}_{\bucket}, \sampleSetTest{\datasetY}_{\bucket}$ at the line \ref{lst:line:permutation-test} computes a p-value given the selected variables $\VariableSelectionHatIndex{\bucket}$, i.e. remaining values at $\VariableSelectionHatIndex{\bucket}$ of $\sampleSetTest{\datasetX}_{\bucket}$ and $\sampleSetTest{\datasetY}_{\bucket}$ and setting all other variables 0.0.
The permutation test requires a distance function for measuring a distance of $\sampleSetTest{\datasetX}_{\bucket}, \sampleSetTest{\datasetY}_{\bucket}$.
The preferred distance function is such as an MMD estimator or Sliced Wasserstein~\citep{bonneel-2015} that measures a distance between two probability distributions.

\begin{algorithm}[tb]
  \caption{
    Time-Slicing Variable Selection
    \newline
    \Comment{
      Input: $X := (x_1,\threeDots,x_{\TimeN}), Y:= (y_1,\threeDots,y_{\TimeN}), X, Y \in \mathbb{R}^{\Dim \times \TimeN}$,
      a set of end time steps of buckets $\{ t_1, \threeDots, t_{\TotalBucketSize} \}$,
      $\ratioTrain$: a ratio of the train set in a bucket,
      $\funcVariableSelection{\cdot}{\cdot}$: a variable selection function.
    }
    \newline
    \Comment{
      Output: $\{ \VariableSelectionHatIndex{\bucketIndex{1}}, \threeDots, \VariableSelectionHatIndex{\bucketIndex{\TotalBucketSize}} \}$:
      A set of selected variables in each bucket.
      $\{ \pValueTest{\bucketIndex{1}}, \threeDots, \pValueTest{\bucketIndex{\TotalBucketSize}} \}$:
      A set of p-values in each bucket.
    }
  }
  \begin{algorithmic}[1]
  \ForAll{b=1,...,\TotalBucketSize}
    \State Randomly split $\IntervalIndex{\bucket}$ such that $\IntervalIndex{\bucket} = \IntervalIndexTrain{\bucket} \cup \IntervalIndexTest{\bucket}$ with a ratio of $\ratioTrain:(1 - \ratioTrain)$. \label{lst:line:define-train-test}
    \State Obtain $\sampleSetTrain{\datasetX}_{\bucket} = \{x_i | i \in \IntervalIndexTrain{\bucket} \}, \sampleSetTest{\datasetX_{\bucket}} =\{x_i | i \in \IntervalIndexTest{\bucket} \}$, similarly for $\sampleSetTrain{\datasetY_{\bucket}}, \sampleSetTest{\datasetY_{\bucket}}$. \label{lst:line:set-X-Y}
    \State Execute the variable selection $\VariableSelectionHatIndex{\bucket} \gets \funcVariableSelection{\sampleSetTrain{\datasetX_{\bucket}}}{\sampleSetTrain{\datasetY_{\bucket}}}$. \label{lst:line:variable-selection}
    \State Permutation test with the selected variables $\pValueTest{\bucket} \gets \funcPermutationTest{\sampleSetTest{\datasetX_{\bucket}}}{ \sampleSetTest{\datasetY_{\bucket}} }{\VariableSelectionHatIndex{\bucket}}$ \label{lst:line:permutation-test}
  \EndFor
  \end{algorithmic}
  \label{alg:time-slicing-variable-selection}
  \end{algorithm}

\paragraph{Example}
\label{sec:example-time-slicing-variable-selection}

Let two time series be $X, Y$ having $\TimeN=130$ time steps and $\Dim=5$.
Figure~\ref{fig:example-time-slicing-iid-idea-a}, \ref{fig:example-time-slicing-iid-idea-b}, \ref{fig:example-time-slicing-iid-idea-c} illustrate examples of dividing the time series of $T=130$ into three buckets.
Suppose that one splits the time steps into $\TotalBucketSize=3$ having 50 steps, i.e. ending steps are $t_{1}=50, t_{2}=100, t_{3}=130$.
The intervals of the buckets are $\IntervalIndex{1}=(0,50], \IntervalIndex{2}=(50,100], \IntervalIndex{3}=(100,130]$.
For each bucket $\bucket \in \{1, 2, 3\}$, one randomly divides $\IntervalIndex{\bucket}$ into $\IntervalIndexTrain{\bucket}$ and $\IntervalIndexTest{\bucket}$ by a ratio of $\ratioTrain=0.8$.
Therefore, $|\IntervalIndexTrain{\bucket}|=40$ and $|\IntervalIndexTest{\bucket}|=10$, and $\sampleSetTrain{\datasetX_{\bucket}}, \sampleSetTest{\datasetX_{\bucket}}$ are sets having 40 and 10 steps that are randomly ordered, similarly for $\sampleSetTrain{\datasetY_{\bucket}}, \sampleSetTest{\datasetY_{\bucket}}$.
Suppose that the variable selection selects two variables $\VariableSelectionHatIndex{\bucket} = \{1, 2\}$ by the $\funcVariableSelection{\sampleSetTrain{\datasetX_{\bucket}}}{\sampleSetTrain{\datasetY_{\bucket}}}$.
These two variables may have responsibilities for rejecting the $H_0$.
To evaluate these selected variables, the permutation test $\funcPermutationTest{\sampleSetTest{\datasetX_{\bucket}}}{\sampleSetTest{\datasetY_{\bucket}}}{\VariableSelectionHatIndex{\bucket}}$ computes a p-value $\pValueTest{\bucket}$,
remaining values at $\VariableSelectionHatIndex{\bucket} = \{1, 2\}$ of $\sampleSetTest{\datasetX_{\bucket}}, \sampleSetTest{\datasetY_{\bucket}}$ and setting all other variables $\hat{S}^c_{\bucket} = \{3, 4, 5\}$ to 0.0.
Suppose that the computed p-value $\pValueTest{\bucket}=0.001$, then these variables $\{1, 2\}$ are with a high probability of discrepancies between $P$ and $Q$, where the significance level is 0.05.
Otherwise, there is a high probability of accepting $H_0$ or these variables $\{1, 2\}$ are not responsible for the discrepancies.
The algorithm iterates the above procedure for $\bucket= 1, 2, 3$ and obtains a set of selected variables $\{\VariableSelectionHatIndex{\bucketIndex{1}}, \threeDots, \VariableSelectionHatIndex{\bucketIndex{3}}\}$ and corresponding p-values $\{\pValueTest{\bucketIndex{1}}, \threeDots, \pValueTest{\bucketIndex{3}}\}$.














\subsection{Limitation of the proposed method}
\label{sec:proposed-method-limitation}

The proposed method is incapable of recognising and distinguishing time series due to the slicing operations.
Figure~\ref{fig:example-time-slicing-iid-idea-b} illustrates this limitation.
The sub-figure on the top represents a monotonically increasing trend during 500 time steps, and the sub-figure on the bottom is a randomly shuffled sequence of the same time series.
These two time series consist of identical values if the temporal order is the same.
However, the two time series of the top and bottom are apparently different sequences.
The proposed method lacks the ability to distinguish these two due to the time-slicing operation.

We exemplify this limitation with an assessment in Section~\ref{sec:experiment-case-2}.
As the assessment demonstrates, there is a possibility of overcoming this limitation by setting a smaller bucket size.
Alternatively, one may consider other statistical testing methods between two time-series such as two sample testing by functional data analysis~\citep{whynne-2022} or multiple testing per selected dimension~\citep{cortes-2020}.
The time-slicing variable selection focuses on the variable selection in case the dimension size is large and hard to conduct manual analysis.
By the combination of the proposed method and other statistical testing methods, one may be able to conduct a comprehensive analysis of the discrepancies between two time series. 

\subsection{Discussion of Two Sample Testing on a small number of Pairs of Time Series}


Model validation and comparison necessitate simulation outputs generated with various random seeds~\citep{law2007simulation}. 
The behaviour of random processes in simulation models varies depending on the random seed, and simulation outputs generated from different random seeds effectively describe the range of possible values. 
Therefore, conducting two-sample testing with a single pair of time series evaluates only one possible outcome of the simulation.

Even though the controversy of this two-sample testing with a single pair of time series, there would be use-cases where a single pair of simulation outputs can lead to a conclusive result. 
In model validation, at least one counterexample can indicate a model's invalidity when a single pair of time series demonstrates the model's invalidity.
For example, Section~\ref{sec:demonstration-particle} exemplifies that a single pair of the simulation and trained DNN model could bring a conclusion saying the DNN model is invalid.

We design the time-slicing variable selection method to work with a single pair of simulation outputs for situations where computationally expensive simulations are limited by budget or when available time series data are scarce. 
The number of simulation outputs used in the algorithm can be adjusted based on the user's preference, allowing for variable selection and two-sample testing with any number of simulation outputs.

We outline the procedure for executing variable selection and computing p-values using multiple pairs of simulation outputs.
Let $N \in \mathbb{N}$ be the number of simulation output pairs, ${(X_1, Y_1),\threeDots,(X_N,Y_N)}$.
First, the time-slicing variable selection of Algorithm~\ref{alg:time-slicing-variable-selection} proceeds for each simulation pair $(X_i, Y_i), i \in \{ 1, \threeDots, N \}$ and obtains a sequence of selected variables $\hat{\mathcal{S}}_{i} = ( \VariableSelectionHatIndex{1},\threeDots,\VariableSelectionHatIndex{B} )$ for the $i$-th pair of simulation output.
When time-slicing variable selection proceeds to all $N$ pairs of simulation outputs, we merge the sequences $\{ \hat{\mathcal{S}}_{1}, \threeDots, \hat{\mathcal{S}}_{N} \}$ per bucket $\bucket$ over $N$ variable selection results.
Let the merged selected variables at bucket $\bucket$ over the above sequences be $\hat{\mathfrak{S}}_b = \{ \VariableSelectionHatIndex{b} \cup \VariableSelectionHatIndex{b}^{(i)} | i \in \{1,\threeDots,N\} \}$.
These selected variables $\hat{\mathfrak{S}}_b$ are variables of being responsible for rejecting $H_0$.


\subsection{Variable Selection Algorithms}
\label{sec:proposal-variable-selection}

We briefly introduce variable selection algorithms that we employ for the proposed method.
Except for Mskernel, these following methods compute a weight vector $w \in \mathbb{R}^{\Dim}$ that represents the importance of each variable, ex. a higher value represents more possibility of having responsibility for rejecting $H_0$.
Given the computed weight vector,
$\VariableSelectionHat$ is selected by a heuristic variable selection method that our previous work~\citep{mitsuzawa-2023} describes in Section 4.2.1.
Hereafter, \textbf{our previous work} refers to \citep{mitsuzawa-2023} if not otherwise stated.


\subsubsection{MMD-Based Variable Selection}
\label{sec:proposal-mmd-based-variable-selection}

Maximum Mean Discrepancy (MMD) is a distance function that measures a distance between two probability distributions~\citep{gretton-2012a}.
In recent studies, MMD is often employed as a distance function of validation of spatial-temporal data, which consists often high dimensional space~\citep{sanchez-2020, Cervellera-2021, feng2023trafficgen}.

The MMD-based variable selection, which is from our previous work, is an optimisation-based variable selection method.
\citep{sutherland2017} proposed to optimise a ARD kernel that is parameterised by ARD weights $a_1,...,a_{\Dim}$.
The optimisation problem aims at maximising an asymptotic approximation of a test power by MMD two-sample testing.
The optimised ARD weights would represent the responsibility level to reject the $H_0$. 
Our previous work pointed out that the optimisation problem may not properly obtain the ARD weights representing responsible variables,
and therefore proposed to regularise the optimisation problem by $L_1$.
The $L_1$ regularised optimisation problem minimises the following objective function:

\begin{equation}
  \label{eq:mmd-optimisation-problem}
  \underset{a \in \mathbb{R}^{\Dim}}{\min} -\log(\ell(a_1,...,a_{\Dim})) + \lambda \sum_{d=1}^{\Dim} |a_d|,
\end{equation}
where the term $\ell(a_1,...,a_{\Dim})$ represents an asymptotic approximation of a test power by MMD two-sample testing.
The $\lambda$ is a hyperparameter of the $L_1$ regularisation, and thus the appropriate $\lambda$ is unknown for the given samples.
Our previous work proposed two methods for seeking the appropriate ARD weights: \emph{MMD Model Selection}~(MMD Model Sel) and \emph{MMD Cross-Validation Aggregation}~(MMD CV AGG).
The first method seeks the most appropriate $\lambda$ that can distinguish the given two samples $\datasetX, \datasetY$, and then regards the obtained ARD weights as the weight vector $w$.
The second method aggregates the ARD weights that are obtained by cross-validations and a set of $\lambda$ candidate parameters and regards the aggregated ARD weights as the weight vector $w$.


\subsubsection{Wasserstein-based Variable Selection}
\label{sec:proposal-wasserstein-based-variable-selection}

The Wasserstein-based variable selection is a heuristic method that computes Wasserstein distances between two samples $\datasetX, \datasetY$ per dimension.
It computes a wasserstein distance per dimension $d \in \{ 1,\threeDots,\Dim \}$,
$$
w_{\rm wass}^d = \text{Wasserstein}(\datasetX^d, \datasetY^d),
$$
where $\datasetX^d, \datasetY^d$ are sets of uni-variate samples at the $d$-th variable $\datasetX^d = \{x^d_1, \threeDots, x^d_n \}, x^d_n \in \mathbb{R}$, similarly for $\datasetY^d$.

Compared to the MMD-based methods, this method lacks considering interactions between variables.
Therefore, it would be possible that this method selects $\VariableSelectionHat$ redundantly.


\subsubsection{Variable Selection by Regularised Regression Models}
\label{sec:proposal-lasso-based-variable-selection}

The two-sample testing problem can be regarded as either a regression problem of estimating two labels $\textbf{L}_{\datasetX}=1.0, \textbf{L}_{\datasetY}=0.0$ or a binary classification problem that classifies the given data into a class of either $\datasetX, \datasetY$.
Thus, a regression model may work for either a regression problem or a binary classification problem, and its explanatory variables may serve as the weight vector $w$.
In case of the regression problem, a regression model $\mathcal{M}$ predicts either $\textbf{L}_{\datasetX}=1.0, \textbf{L}_{\datasetY}=0.0$,
$$
\mathcal{M} = \beta_0 + \sum_{d=1}^{D}\beta_{d} \phi_{d},
$$
where $\phi_d$ is a value of given samples from either $\datasetX$ or $\datasetY$ and $\beta_d$ is the explanatory variable.
An elastic net~\citep{zou-2005} is a regression model equipped with $L_1$, $L_2$ terms of regularising the explanatory variables.
The regression model minimises the following objective function,

$$
\underset{B \in \mathbb{R}^{D}}{min} \sum_{i=1}^{n} (y_i - \mathcal{M}(x_i))^2 + \lambda_1 \sum_{d=1}^{D} |\beta_d| + \lambda_2 \sum_{d=1}^{D} \beta_d^2,
$$
where $\lambda_1, \lambda_2$ are hyperparameters of the $L_1$ and $L_2$ regularisation respectively.
When $\lambda_2$ is 0.0, the regression model is a lasso regression model and a ridge regression model when $\lambda_1$ is 0.0.
Once the model fits the given data, we regard the explanatory variables as the weight vector $w$.

For the binary classification problem, we employ a logistic regression model that predicts a binary label either $\textbf{L}_{\datasetX}=1$ or $\textbf{L}_{\datasetY}=0$. 

We seek the most appropriate hyperparameters $\lambda_1, \lambda_2$ with two strategies of parameter searching: \emph{Regression-Fit} and \emph{Regression-P-value}.
The Regression-Fit strategy attempts to maximise a fitting score $R^2$ of a regression model.
The Regression-P-value strategy attempts to minimise the p-value of a permutation test computed with the selected variables;
First, we split the given dataset into a train and development set, and the variable selection task is executed with the train set and obtains $\VariableSelectionHatIndex{\rm train}$, finally, the permutation test computes a p-value on the development set.
Please refer to Appendix~\ref{sec:appendix-regression-model-hyperparameter} for the details of the hyperparameter searching procedure.

Compared to the MMD-based methods, this variable selection method does not consider the non-linearity.
Moreover, the objective function is incapable of explicitly handling the two-sample testing problem.
The regression-p-value strategy can not solve the variable selection task for two-sample testing in the closed form due to the permutation test.
Therefore, this variable selection method would be applicable in only limited cases.

\subsubsection{Mskernel-star}
\label{sec:proposal-mskernel-variable-selection}

\emph{Mskernel}~\citep{Lim-2020}\footnote{We use the codebase by the authors \href{https://github.com/jenninglim/multiscale-features}{\url{https://github.com/jenninglim/multiscale-features}}. \emph{Mskernel} names after the codebase and \emph{star} represents that the Mskernel algorithms knows the expected number of variables.} is a variable selection method powered by the post-selection inference and tests by MMD estimate.

Compared to other methods, the Mskernel-start requires the expected number of variables as a hyperparameter.


==> experiment_records.tex <==

\section{Experiment Record}

All contents in this sections from here, all unofficial \texttwemoji{smile}.


































































\subsection{Synthetic Simpler Setting}
\label{sec:synthetic-data-setting}

$T$ is a set of time-step. 
$t \subset T$ is a time-step, $0 < t < 1$. 
A sequence of $t$ has spans with equal values.

The data generation function generates $X = \{x_1,...,x_t\}, x_t \in \mathbb{R}^{D}, d \subset D, d > 0$.
The function generates $x_t$ at a time-step $t$ with

\begin{equation}
\begin{split}
x^1(t) & = t + \epsilon^1_t \\
& ... \\
x^d(t) & = t + \epsilon^d_t
\end{split}
\end{equation}.

I define $\epsilon \sim P$.

The data generation function generates $Y = \{y_1, ..., y_t \}, y_t \in \mathbb{R}^{D}, d \subset D, d > 0$.
The function generates $y_t$ at a time-step $t$ with

\subsubsection{Noising: standard scenario}
\label{sec:noising-standard-scenario}

The code-name is \verb|standard|.

I define two variable types; normal and noised.
The normal variables follow always $y^d(t) = t + \Tilde{\epsilon}^d_t, t = [0, 1.0]$.
The noised variable follows the following generation process,

\begin{equation}
    \begin{split}
        y^1(t) & = \begin{cases}    
            t_{\rm perturbation\ start} + \Tilde{\epsilon}^1_t, & \text{if $t_{\rm perturbation\ start} \leq t \leq t_{\rm perturbation\ end}$} \\
            t + \Tilde{\epsilon}^1_t, & \text{otherwise}.
        \end{cases}, \\
        & ..., \\
        y^d(t) & = t + \Tilde{\epsilon}^d_t
    \end{split}
\end{equation}.

An example visualizations are at Figure~\ref{fig:visualization-noising-standard}.

\begin{figure}[th]
  \begin{subfigure}{.5\textwidth}
  \centering
    \includegraphics[width=0.5\linewidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/figure-standard/data-noised-agents.png}
    \caption{Noised dimensions}
  \end{subfigure}%
  \begin{subfigure}{.5\textwidth}
  \centering
    \includegraphics[width=0.5\linewidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/figure-standard/data-non-noised-agents.png}
    \caption{Dimension without noise}
  \end{subfigure}
  \caption{Code name: \emph{standard}. See Section \ref{sec:noising-standard-scenario}. $P=Q=N(\mu, \sigma^2), \mu=0, \sigma=0.1$}
  \label{fig:visualization-noising-standard}
\end{figure}



\subsubsection{Noising: inversed scenario}
\label{sec:noising-inversed-scenario}


The code-name is \verb|inversed|.

\begin{equation}
    \begin{split}
        y^1(t) & = \begin{cases}    
            t_{\rm perturbation\ end} - (t - t_{\rm perturbation\ stard}) + \Tilde{\epsilon}^1_t, & \text{if $t_{\rm perturbation\ start} \leq t \leq t_{\rm perturbation\ end}$} \\
            t + \Tilde{\epsilon}^1_t, & \text{otherwise}.
        \end{cases}, \\
        & ..., \\
        y^d(t) & = t + \Tilde{\epsilon}^d_t
    \end{split}
\end{equation}.

An example. Figure~\ref{fig:visualization-noising-inversed}.


\begin{figure}[th]
  \begin{subfigure}{.5\textwidth}
  \centering
    \includegraphics[width=0.5\linewidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/figure-inversed/data-noised-agents.png}
    \caption{Noised dimensions}
  \end{subfigure}%
  \begin{subfigure}{.5\textwidth}
  \centering
    \includegraphics[width=0.5\linewidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/figure-inversed/data-non-noised-agents.png}
    \caption{Dimension without noise}
  \end{subfigure}
  \caption{Code name: \emph{inversed}. See Section \ref{sec:noising-inversed-scenario}. $P=Q=N(\mu, \sigma^2), \mu=0, \sigma=0.1$}
  \label{fig:visualization-noising-inversed}
\end{figure}

\subsubsection{Generation Parameters}















 







\subsubsection{Detection Record}












\subsubsection{Log 2024-03-07}
\label{sec:2024-03-07}

The detection is for \verb|standard|, Sec \ref{sec:noising-standard-scenario}, noising case only, in Fig~\ref{fig:visualization-noising-standard}.
One data iteration.
$\mathbb{R}^{D}, D=5$.
One dimension has the noise.
The noise vector index is always $1$\footnote{Counting it with 0-index style.}.

Time steps are in $0.001$ interval, so $\{0.001, 0.011, 0.021, ..., 1.0\}$.
The total steps are 999 steps.
The noising during $[1/4, 1/2]$.
3 configurations of time-bucket size, $|\mathcal{B}|$, $\{100, 300, 500\}$.

\texttwemoji{paperclip} Quick Conclusion. \textcolor{brown}{MMD CV-AGG}, \textcolor{pink}{MMD Selection} are the best method in this trial. Although, these two failed at the noise starting point task at Time-Slicing=100 (See \ref{fig:2024-03-07-p-values}), others are all perfect (See variable detection Fig~\ref{fig:2024-03-07-variable-detection-at-prediction}). 

\texttwemoji{pencil}: Observation and subjective comments per method.

\textcolor{violet}{Baseline MSKernel} failed to select any variables in all cases. The first step fails. Variable selection scores are also all 0.0. \verb|MSKernel| selects variables in 2-steps; selecting candidate variables by somehow heuristic method, and then evaluating p-value for each candidate. I wonder my configuration would not be correct? \texttwemoji{thinking}. I follow author's example code though.

\textcolor{blue}{Baseline Regression-Fit} and \textcolor{orange}{Baseline Regression-P} are, interestingly, detected the noise-starting bucket at Time-Slicing=100, even though proposal methods failed to detect \texttwemoji{flushed}.
The reason is unknown, for the moment.
Looking at evaluation scores of variable detection at the case of Time-Slicing=100, \emph{Recall} scores are always 1.0.
On the other hand, \emph{Precision} is around 0.3, which means detecting 3 variables.
Same as in the TPAMI submission; Regression based methods select too much variables.

\textcolor{red}{Baseline MMD} correctly detected the noise-starting bucket at Time-Slicing=100.
Yet, the evaluation score of variable detection is 0.0.
This is due to non-regularised optimization. 
In fact, the optimized ARD weights at time-bucket-index=2 is \mintinline{Python}{[0.5503514409065247, 0.16681614518165588, 0.3461233079433441, 0.22494839131832123, 0.8182010054588318]}, then detected variables are \mintinline{Python}{[0, 2, 3, 4]}\footnote{The truth is variable 1.}.
\verb|Baseline MMD| does optimization for maximizing a test-power with caring differences between sample sets $X, Y$.
I may address this drawback of MMD Baseline as strong motivation of using proposal methods \texttwemoji{+1}.
Looking at Fig~\ref{fig:2024-03-07-variable-detection-at-truth}, Baseline MMD is able to discover noised variables when the it knows the ground-truth of the noise starting point.
Although, the evaluation scores low precisions, high recall, which means Baseline MMD selects too much variables.

\textcolor{green}{Baseline Wasserstein}, \textcolor{brown}{MMD CV-AGG}, \textcolor{pink}{MMD Selection}, these 3 methods are in similar tendencies.
Yet, a different is at Time-Slicing=300.
First, I describe comparison at Time-Slicing=300.

Looking at Fig~\ref{fig:2024-03-07-p-values}, \textcolor{green}{Baseline Wasserstein} failed to detect the noise starting point, whereas two MMD based proposal correctly detected the noise starting point.
This is because \textcolor{green}{Baseline Wasserstein} selected too much variables.
Please look at Fig~\ref{fig:2024-03-07-variable-detection-at-truth}, \textcolor{green}{Baseline Wasserstein} made the lower precision score and 1.0 recall score at Time-Slicing=300\footnote{Actually, 4 variables selected out of 5.}.
Due to too much selected variables, a permutation test accepted $H_0$.
\texttwemoji{blush}: a drawback of \textcolor{green}{Baseline Wasserstein} compared to MMD based proposals.
\texttwemoji{thinking}: Maybe due to available samples. Need to validate this tendency with other sample sets.




\paragraph{Detection Settings}
\label{sec:2024-03-07-detection-settings}

Data splitting.
$Train:Test=0.8:0.2$, randomly selected.
Note that the the current codebase has two non-deterministic behaviours.
The one is at splitting time steps for either train:test or train:dev.
The second is in the permutation test. 
The permutation shuffling is non-derterministic.
Hence, the code execution results are not 100\% same.

Baseline MMD's configuration is below.
One MMD-Opt is with upper-bound of 5000 epochs.
Two Early-Stoppers \verb|ConvergenceEarlyStop| and \verb|VariableEarlyStopping|, see the next paragraph for the details.
Adam Optimizer, the initial learning rate is 0.01.
Reducing to 0.001 lower bound, monitoring the loss value.

\verb|ConvergenceEarlyStop| and \verb|VariableEarlyStopping| are early stoppers of optimization.
\verb|ConvergenceEarlyStop| monitors the loss value\footnote{by default, possible to change} and forces to stop the optimization when $min(v)/max(v) < 0.001$ among 100 epochs window-span, where $v$ is the target of monitor, the loss value in this case.
\verb|ConvergenceEarlyStop| does not activate during the first 500 epochs.
\verb|VariableEarlyStopping| monitors the discretized set of variables $D_{\rm select}$ and forces to stop the optimization when $D_{\rm select}$ are same during 100 epochs window-span.
\verb|VariableEarlyStopping| ignores the first 300 epochs.
\verb|VariableEarlyStopping| is necessary from experiences.
In optimizing with practical data, there are cases where the loss value do not converge under the condition of $min(v)/max(v) < 0.001$, in other words, loss value keep going smaller\footnote{recall minimization problem.}.
Our primary target is variable selection/detection, hence precise MMD-Opt is not mandatory, rather satisfied when the selected variables are "converged".


Baseline Regression's configurations.
5 Fold-cross validation\footnote{Fold validation operation is by \emph{Scikit-learn}}.
Per each fold, Optuna does hyper-parameter optimization problem up to 20 trials.
For computational efficiency, Dask\footnote{Python-native distributed computing platform} lets 5 regression models fit in parallel.
Optuna receives objective value of 5 regression models, and proposes a set of 5 new hyper-parameters of regression models.
Hence, 4 times hyper-parameter updates considering 5 trials in the same time.

Baseline Mskernel follows the example code at \href{https://github.com/jenninglim/multiscale-features/blob/master/notebooks/anomaly%20dataset%20detection.ipynb]}{Author's notebook}.


MMD CV-AGG... $|\Lambda| = 5$, $N_{\rm CV}=6$.
$\lambda_{\rm lower}$ and $\lambda_{\rm upper}$ is by Optuna search.
The Optuna's objective function is $|D_{\rm select}|$.
Minimization problem for $\lambda_{\rm upper}$,
Maximization problem for $\lambda_{\rm lower}$.
The MMD-Opt configurations are the same as Baseline MMD.


MMD Selection... $|\Lambda| = 10$. 
The $\lambda$ parameter selection is done by Optuna. 
Optuna's objective function is $r_{\rm test\ power\ dev} + (1 - p_{\rm dev})$. 
Optuna solves the maximization problem.
$|\Lambda| = 10$ is equal to the iteration number of parameter searching of Optuna.
The MMD-Opt configurations are the same as Baseline MMD.





\paragraph{P-value Sequence}

Fig~\ref{fig:2024-03-07-p-values} represents the results of noise-starting point detection.


\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/p_value_sequence/pvals-standard-noise-100-steps.toml-data-0.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/p_value_sequence/pvals-standard-noise-300-steps.toml-data-0.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/p_value_sequence/pvals-standard-noise-500-steps.toml-data-0.png}
        \caption{P-values and Time-Buckets. Time-Bucket size $\{100, 300, 500\}$ from the left. Color lines represent variable selection methods. The red dot line in the vertical axis is at $0.05$ of rejecting $H_0$ hypothesis. The blue star marker is the ground-truth time-bucket of noise-starting point.
        Traceback to \ref{sec:2024-03-07}.}
        \label{fig:2024-03-07-p-values}
    \end{figure*}
\end{multicols}


\paragraph{Variable Detection at $H0$ rejection bucket}

Fig~\ref{fig:2024-03-07-variable-detection-at-prediction}.
Table~\ref{tab:2024-03-07-result-table}.

\begin{multicols}{3}
    \begin{figure*}
        \centering
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/var_detection_detection/Precision.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/var_detection_detection/Recall.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/var_detection_detection/F.png}
        \caption{Evaluation scores of variable detection. \emph{Precision, Recall, F} from the left. The horizontal axis labels are time-slicing size, which is $\{100, 300, 500\}$ from the left. Score is $0.0$ when p-value > 0.05 for all time-buckets. Please refer to Fig~\ref{fig:2024-03-07-p-values}. Traceback to \ref{sec:2024-03-07}}
        \label{fig:2024-03-07-variable-detection-at-prediction}
    \end{figure*}
\end{multicols}

\begin{table}
\fontsize{6}{7}\selectfont
\begin{tabular}{p{2cm} | p{1cm} | p{2cm} | p{1cm} | p{1cm} | p{0.9cm} | p{0.9cm} | p{0.15cm} | p{0.15cm} | p{0.15cm}}
    \centering
    \setlength{\tabcolsep}{0.11cm}
    $|\mathcal{B}|$ & data-id & Method & Predicted $\mathcal{B_{\rm noise\ start}}$ & True $\mathcal{B_{\rm noise\ start}}$ & $\rho_{\rm pred}$ & $\rho_{*}$ & P & R & F \\
    \midrule
    Time-Slicing=100 & data-0 & Baseline MMD & 3 & 3 & 0.5 & 0.5 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=100 & data-0 & Baseline MsKernel & -1 & 3 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=100 & data-0 & Baseline Regression-Fit & 3 & 3 & 0.5 & 0.5 & 0.3 & 1.0 & 0.5 \\
    Time-Slicing=100 & data-0 & Baseline Regression-P & 3 & 3 & 0.5 & 0.5 & 0.2 & 1.0 & 0.4 \\
    Time-Slicing=100 & data-0 & Baseline Wasserstein & 4 & 3 & 1.0 & 0.5 & 1.0 & 1.0 & 1.0 \\
    Time-Slicing=100 & data-0 & MMD CV-AGG & 4 & 3 & 1.0 & 0.5 & 0.5 & 1.0 & 0.7 \\ 
    Time-Slicing=100 & data-0 & MMD Selection & 4 & 3 & 1.0 & 0.5 & 1.0 & 1.0 & 1.0 \\ \hline
    Time-Slicing=300 & data-0 & Baseline MMD & -1 & 2 & 0.0 & 0.7 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=300 & data-0 & Baseline MsKernel & -1 & 2 & 0.0 & 0.7 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=300 & data-0 & Baseline Regression-Fit & 4 & 2 & 0.0 & 0.7 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=300 & data-0 & Baseline Regression-P & -1 & 2 & 0.0 & 0.7 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=300 & data-0 & Baseline Wasserstein & -1 & 2 & 0.0 & 0.7 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=300 & data-0 & MMD CV-AGG & 2 & 2 & 0.7 & 0.7 & 1.0 & 1.0 & 1.0 \\
    Time-Slicing=300 & data-0 & MMD Selection & 2 & 2 & 0.7 & 0.7 & 1.0 & 1.0 & 1.0 \\ \hline
    Time-Slicing=500 & data-0 & Baseline MMD & -1 & 1 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=500 & data-0 & Baseline MsKernel & -1 & 1 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=500 & data-0 & Baseline Regression-Fit & -1 & 1 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=500 & data-0 & Baseline Regression-P & -1 & 1 & 0.0 & 0.5 & 0.0 & 0.0 & 0.0 \\
    Time-Slicing=500 & data-0 & Baseline Wasserstein & 1 & 1 & 0.5 & 0.5 & 1.0 & 1.0 & 1.0 \\
    Time-Slicing=500 & data-0 & MMD CV-AGG & 1 & 1 & 0.5 & 0.5 & 1.0 & 1.0 & 1.0 \\
    Time-Slicing=500 & data-0 & MMD Selection & 1 & 1 & 0.5 & 0.5 & 1.0 & 1.0 & 1.0 \\
\end{tabular}
\caption{Variable detection result. P: Precision, R: Recall. Evaluation scores are at a time-bucket $\mathcal{B}$ where the smallest index of method rejected $H_0$. $-1$ at "Predicted $\mathcal{B_{\rm noise\ start}}$" represents accepting $H_0$ for all. $\rho$ represents a ratio of $|T_{\rm noise}| / |T|$ at a bucket. Traceback to \ref{sec:2024-03-07}}
\label{tab:2024-03-07-result-table}
\end{table}


\paragraph{Variable Detection at the Ground-Truth}

Fig~\ref{fig:2024-03-07-variable-detection-at-truth}.

\begin{multicols}{3}
    \begin{figure*}
        \centering
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/var_detection_truth/Precision.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/var_detection_truth/Recall.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-standard/visualizations/var_detection_truth/F.png}
        \caption{Evaluation scores of variable detection at the ground-truth where the noising starts. Score is $0.0$ when p-value > 0.05 at the ground-truth time-bucket. All other descriptions are the same as at Fig~\ref{fig:2024-03-07-variable-detection-at-prediction}. Traceback to \ref{sec:2024-03-07}.}
        \label{fig:2024-03-07-variable-detection-at-truth}
    \end{figure*}
\end{multicols}


\subsubsection{Log 2024-03-09}
\label{sec:2024-03-09}

The noising setting is \verb|inversed|, Sec~\ref{sec:noising-inversed-scenario}. 
\hypertarget{2024-03-09-tst-failure-assumption}{Firstly,} I address that all methods are expected to detect the noise starting point correctly.
This assumption is due to destroy the time-series structure as in Fig~\ref{fig:example-time-slicing-iid}.

Configurations of methods are all the same as in Sec~\ref{sec:2024-03-07-detection-settings}.

Quick index to Figures. P-value sequence in Fig~\ref{fig:2024-03-09-p-values}, evaluation for var. detection at the predicted time-bucket in Fig~\ref{fig:2024-03-09-variable-detection-at-prediction}, evaluation for var. detection at the truth time-bucket in Fig~\ref{fig:2024-03-09-variable-detection-at-truth}.

\paragraph{Noise Starting Point Detection}

First, \hypertarget{2024-03-09-bucket-100-p-value}{analysis of noise starting point detection} in Fig~\ref{fig:2024-03-09-p-values}.
Against the assumption of failures, methods successfully detected the noise starting point at bucket size $\{100, 300\}$.
That is due to the relations of noise time steps and the separation of time buckets.
Fig~\ref{fig:2024-03-09-error-illustration} explains the reason.
Taking a case of bucket size 100, the noising starts in the 2nd time bucket.
Then, \textcolor{blue}{the noise samples} (colour according to the Figure) are with huge values, compared with \textcolor{red}{non-noised samples}.
Therefore, some methods reject $H_0$ at the 2nd time bucket.
At the 3rd time bucket, two lines are really in opposite directions.
When splitting a line into independent samples, two lines are similar sets of samples.
Therefore, all methods accept $H_0$.
At the 4th bucket, \textcolor{blue}{noise line} are with low values compared to \textcolor{red}{non-noised line}.
Therefore, methods reject $H_0$.

At the 3rd time bucket in the bucket size 100, even \emph{Baseline Regression P} successfully rejects $H_0$.
Considering this result, the two-sample testing problem is quite easy at the 3rd time bucket. 

The same phenomenon is supposed to be at the first time bucket in bucket size 300 case.

At the time bucket 500 case, all methods failed to reject $H_0$ at the 1st time bucket.
This follows \protect\hyperlink{2024-03-09-tst-failure-assumption}{the failure assumption}.  
Splitting time-series into a set of independent samples, hence all methods are not able to recognize shapes of time-series.





\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/p_value_sequence/pvals-inverse-noise-100-steps.toml-data-0.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/p_value_sequence/pvals-inverse-noise-300-steps.toml-data-0.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/p_value_sequence/pvals-inverse-noise-500-steps.toml-data-0.png}
        \caption{P-values and Time-Buckets. Time-Bucket size $\{100, 300, 500\}$ from the left. Color lines represent variable selection methods. The red dot line in the vertical axis is at $0.05$ of rejecting $H_0$ hypothesis. The blue star marker is the ground-truth time-bucket of noise-starting point. Traceback to \ref{sec:2024-03-09}.}
        \label{fig:2024-03-09-p-values}
    \end{figure*}
\end{multicols}


\begin{multicols}{1}
    \begin{figure*}
        \centering
        \includegraphics[width=1.0\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/illustrations/illustration-inverse-noise-02.png}
        \caption{Additional explanation of Fig.~\ref{fig:2024-03-09-p-values}. The \textcolor{red}{red line} is a sample set from $P$, \textcolor{blue}{blue line} is a sample set from $Q$. The \textcolor{green}{green lines} are separations of time buckets. See \protect\hyperlink{2024-03-09-bucket-100-p-value}{this description} for more.}
        \label{fig:2024-03-09-error-illustration}
    \end{figure*}
\end{multicols}


\begin{multicols}{3}
    \begin{figure*}
        \centering
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/var_detection_detection/Precision.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/var_detection_detection/Recall.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/var_detection_detection/F.png}
        \caption{Evaluation scores of variable detection. \emph{Precision, Recall, F} from the left. The horizontal axis labels are time-slicing size, which is $\{100, 300, 500\}$ from the left. Score is $0.0$ when p-value > 0.05 for all time-buckets. Please refer to Fig~\ref{fig:2024-03-09-p-values}. Traceback to \ref{sec:2024-03-09}}
        \label{fig:2024-03-09-variable-detection-at-prediction}
    \end{figure*}
\end{multicols}


\begin{multicols}{3}
    \begin{figure*}
        \centering
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/var_detection_truth/Precision.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/var_detection_truth/Recall.png} \hfil
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_67/5-dims/noise-inverse/visualizations/var_detection_truth/F.png}
        \caption{Evaluation scores of variable detection at the ground-truth where the noising starts. Score is $0.0$ when p-value > 0.05 at the ground-truth time-bucket. All other descriptions are the same as at Fig~\ref{fig:2024-03-09-variable-detection-at-prediction}. Traceback to \ref{sec:2024-03-09}.}
        \label{fig:2024-03-09-variable-detection-at-truth}
    \end{figure*}
\end{multicols}


\subparagraph{Technical Note: \emph{MSkernel}}
\label{sec:technical-note-mskernel}

This paragraph describes why MSkernel dramatically fails.

Simply say, \verb|Mskerel| selects variables in two steps; 1. Selecting top K-variables based on a kernel matrix, 2. Executing MMD-based-two-sample-testing for the selected top-k variables.
If the 1st step fails to select expected variables, \verb|Mskernel| is not able to select expected variables anymore.

I validate this error by codebase.
A class of the feature selection is at \verb|MultiSel|, \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/mskernel/featsel.py#L37C7-L37C15}{on codebase}.
\verb|MultiSel| computes kernel matrices at \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/mskernel/featsel.py#L56-L60}{these lines}, the author left comments saying \emph{"Compute mean and variance of covariance matrix"}.
The actual codebase of computing kernel matrices is at \verb|MMD_Inc| class, \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/mskernel/mmd.py#L13}{on codebase}.
Then, the codebase jumps into \verb|estimates()| method where the \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/mskernel/mmd.py#L50C9-L50C18}{codebase}.

The \verb|estimates()| method, \textbf{seems to be}, computes MMD estimate.
The process flow follows as
\begin{enumerate}
    \item computing kernel matrices $k(X, X), k(Y, Y), k(X, Y)$, \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/mskernel/mmd.py#L58-L60}{lines}.
    \item computing \verb| Kxx[i][j]+ Kyy[i][j] - Kxy[j][i]  - Kxy[i][j]|. This line seems to compute MMD.
    \item returning \verb|sample| which is a vector of $\mathbb{R}^{|D|}$, where $|D|$ is the number of variables.
\end{enumerate}

After the method \verb|estimates()|, as I describe below, the codebase selects the top-k variables having high MMD estimate values.
And then, the codebase executes a sample test for the selected variables.

The drawback is, as I describe before, the 2-steps procedures.
When the 1st step of computing MMD estimates fails to select variables, the codebase is not able to select discarded variables anymore.

I guess that a problem is that the kernel function is not proper of computing MMD estimate.
Therefore, the codebase would fail to compute correct MMD estimate values.

For the information, I leave an investigation note.
The kernel function is \verb|KIMQ| class, which is an inverse multiquadric (IMQ) kernel, \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/mskernel/kernel.py#L158}{here}.
The kernel function is from "Measure Sample Quality with Kernels", Jackson Gorham, Lester Mackey.
The EQ is \verb|k(x,y) = (c^2 + ||x-y||\^2)\^b| according to the author's comment, where \verb|the paper sets b = -1/2 and c = 1|.

The paper used a Gaussian kernel, \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/experiments/exp1a.py#L26-L27}{lines}.
But, \href{https://github.com/jenninglim/multiscale-features/blob/master/notebooks/anomaly%20dataset%20detection.ipynb}{the notebook} used IMQ kernel.
No idea why he used IMQ kernel for the notebook, which is a demonstration case.
For the fare comparison, I should show results with a Gaussian kernel.

=================================================================================

I run the experiment code in the setting of Sec~\ref{sec:2024-03-07} with Gaussian Kernel.
I used author's code for computing $\sigma$ length-scale parameter, \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/experiments/exp1a.py#L26}{codebase}.
The length-scale computation seems to be the median-heuristic.
Nothing different.
The 1st step of \verb|Mskernel| detected incorrect variables, and then p-values > 0.05 for all selected at the 2nd steps, of course.
In the end, no variables detected.

From this result, I guess that kernel length scale play a important role.
A median heuristic length scale seems not be able to obtain a robust kernel function.

Another possibility is the amount of samples.
Looking at experiment codes of \verb|Mskernel|, the sample sizes are $\{500, 1000, 1500, 2000\}$, ex. \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/experiments/exp1a.py#L21}{here} where the dimension is \href{https://github.com/jenninglim/multiscale-features/blob/54b3246cf138c9508e92f466e25cc4e778d0728a/experiments/exp1a.py#L160}{50}.

The \verb|Mskernel| codebase may work well if it executes two-sample testing to all variables.
In other words, I skip the 1st step.
But, for the moment, the codebase is not able to do easily.
So, I simply give up doing so.
Not scope of my work.


\subsubsection{Logs 2024-03-12}
\label{sec:2024-03-12}

Assessment, following a feature plan in \href{https://codehub-g.huawei.com/k50037225/mmd-tst-variable-detector/issues/84}{on CodeHub}.

\paragraph{Summary}

Synthetic data generation: Sec~\ref{sec:synthetic-data-setting}.
5 dimension. 1 noised dimension.

3 iterations of data-generations and experiments run.
Different random seed for each data-generation and run.
I visualize the generated data in Fig~\ref{fig:2024-03-12-data-visualization}.

Detection methods: Sec~\ref{sec:2024-03-07-detection-settings}.


\begin{figure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/data-visualization/data-0.png}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/data-visualization/data-1.png}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/data-visualization/data-2.png}
    \end{subfigure}
    \caption{
    Synthetic generated time-series in 3 iterations; each column, one data.
    The upper rows are time-series of noised-dimension.
    The blue dashed-lines are time spans where the noise exists.
    The bottom rows are one of time-series without the noise.
    Traceback to \ref{sec:2024-03-12}.
    }
    \label{fig:2024-03-12-data-visualization}
\end{figure}


\paragraph{Breaking change: Evaluation}

An major update in evaluation.


$$
{\rm Precision} = \frac{|D_{\rm select} \cap D^*|}{|D_{\rm select}|}
$$

$$
{\rm Recall} = \frac{|D_{\rm select} \cap D^*|}{|D^*|}
$$

$$
{\rm F} = \frac{2 * {\rm Precision} * {\rm Recall}}{{\rm Precision} + {\rm Recall}}
$$

$D_{\rm select}$ is a set of variables by a method.
$D^*$ is a set of ground-truth of the noised variable.

Definitions of $D_{\rm select}, D^*$ varies either \emph{evaluation at $H_0$ rejection} or \emph{evaluation at ground-truths}.

When \hypertarget{2024-03-12-eval-rejection}{the evaluation at $H_0$ rejection}, $D_{\rm select} := D_{p(\mathcal{B}) \leq 0.05}$ is a set of variables where the p-value <= 0.05 \textbf{first time}, and $D^* := D^*_{p(\mathcal{B}) \leq 0.05}$ is a set of ground-truth variable at a time-bucket where a p-value of a method is less than 0.05 first time. 
$p(\mathcal{B})$ represents a p-value at a time bucket. 
\textbf{Evaluation score is zero} when a method has no time buckets with p-value <= 0.05.


When \hypertarget{2024-03-12-eval-truth}{evaluation at ground-truth}, $D_{\rm select} := D_{\rm select_{\mathcal{B}^*}}$ is variables in \textbf{a set of noised time bucket} and $D^* := D^*_{\mathcal{B}^*}$ is ground-truth variables at \textbf{a set of ground truth time buckets} where the noised variables exist.
This evaluation is regardless of p-value at $\mathcal{B}^*$; I compute evaluation score even though p-vale > 0.05.

Even though the definition is different, $D^*$ is \textbf{the same set} in this assessment.
The purpose of "evaluation at ground-truth" is to understand variable influences on p-value.
If the variable selection is correct, then p-value should be <= 0.05.

\paragraph{Minor Change: Mskernel-Gaussian}

Investigation Sec~\ref{sec:technical-note-mskernel}.
Then, I found that the author's code used a IMQ kernel while his paper used a Gaussian kernel, weird inconsistency \texttwemoji{thinking}.
For the fare comparison, I evaluated "Baseline MsKernel" with a gaussian kernel. 


\paragraph{Result}

P-value sequence Fig~\ref{fig:2024-03-12-p-values}.
Table~\ref{tab:2024-03-12-p-value-agg}.

Variable detection. Fig~\ref{fig:2024-03-12-variable-detection-at-prediction} and Fig~\ref{fig:2024-03-12-variable-detection-at-truth}.

\paragraph{Analysis}

\texttwemoji{blush} I am happy.
The proposal \textcolor{gray}{MMD CV-AGG} is the most stable method. 
Permutation test results are positive; accurate $H_0$ rejections at "Time-Slicing=300" and "Time-Slicing=500" Fig~\ref{fig:2024-03-12-p-values}.
The variable detection results are also most stable -> Fig~\ref{fig:2024-03-12-variable-detection-at-prediction}.

\hypertarget{2024-03-12-analysis-self-comment}{Self-comment} to Fig~\ref{fig:2024-03-12-variable-detection-at-truth};
At "Time-Slicing=100", \textcolor{gray}{MMD CV-AGG} and \textcolor{olive}{MMD Selection} show lower precision and f scores.
This is because detected variables at time-bucket=3.
At time-bucket=3, both two methods accepted $H_0$ which is false-negative, see Fig~\ref{fig:2024-03-12-p-values} \footnote{Type-II error with a term of two sample testing.}.
This false-negative is because both two methods selected too much variables.
Recall that the evaluation at Fig~\ref{fig:2024-03-12-variable-detection-at-truth} evaluates all variables at time-buckets $\{3, 4, 5\}$.
Since too much incorrect selected variables at time-bucket=3, the precision score goes down. 
So, why variable selection failed at the time-bucket=3?
\texttwemoji{thinking} I guess due to \textbf{noisy and fewer} sample size.
The "Time-Slicing=100" setting has $|\mathcal{B}| = 100$,
Among 100 samples, the noised samples are only 50 samples.
And splitting 80 samples for training and 20 for testing\footnote{the splitting is random selection.}.
Would be, too few sample size for detecting noised variables.


\textcolor{blue}{Comment: Time-bucket=100, bucket-index=9. Why rejection? Need to check.}


\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/p_value_sequence_aggregation/pvals-standard-noise-100-steps.toml.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/p_value_sequence_aggregation/pvals-standard-noise-300-steps.toml.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/p_value_sequence_aggregation/pvals-standard-noise-500-steps.toml.png}
        \caption{
        Aggregated P-values and Time-Buckets. 
        Time-Bucket size $\{100, 300, 500\}$ from the left. 
        3 iterations. 
        Color lines represent the average p-value for variable selection methods. 
        The color region is std values. 
        The red dot line in the vertical axis is at $0.05$ of rejecting $H_0$ hypothesis. 
        The blue stars are the ground-truth time-bucket of noise-starting point. 
        Traceback to \ref{sec:2024-03-12}.}
        \label{fig:2024-03-12-p-values}
    \end{figure*}
\end{multicols}


\begin{table}[ht]
    \centering
    \fontsize{6}{7}\selectfont
    \begin{tabular}{ p{2cm} | p{1cm} | p{2.5cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} }
    \toprule
    $|\mathcal{B}|$ & $\mathcal{B}_i$ & Method & $avg(p)$ & $std(p)$ & $min(p)$ & $max(p)$ \\
    \midrule
    Time-Slicing=100 & 3 & Baseline MMD & 0.587 & 0.517 & 0.002 & 0.982 \\
    Time-Slicing=100 & 3 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 3 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 3 & Baseline Regression-Fit & 0.309 & 0.276 & 0.004 & 0.542 \\
    Time-Slicing=100 & 3 & Baseline Regression-P & 0.320 & 0.249 & 0.032 & 0.468 \\
    Time-Slicing=100 & 3 & Baseline Wasserstein & 0.357 & 0.055 & 0.294 & 0.391 \\
    Time-Slicing=100 & 3 & MMD CV-AGG & 0.657 & 0.084 & 0.592 & 0.752 \\
    Time-Slicing=100 & 3 & MMD Selection & 0.795 & 0.196 & 0.570 & 0.932 \\
    Time-Slicing=100 & 4 & Baseline MMD & 0.716 & 0.169 & 0.588 & 0.908 \\
    Time-Slicing=100 & 4 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 4 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 4 & Baseline Regression-Fit & 0.511 & 0.110 & 0.390 & 0.606 \\
    Time-Slicing=100 & 4 & Baseline Regression-P & 0.481 & 0.066 & 0.418 & 0.550 \\
    Time-Slicing=100 & 4 & Baseline Wasserstein & 0.047 & 0.080 & 0.001 & 0.140 \\
    Time-Slicing=100 & 4 & MMD CV-AGG & 0.002 & 0.000 & 0.002 & 0.002 \\
    Time-Slicing=100 & 4 & MMD Selection & 0.009 & 0.012 & 0.002 & 0.022 \\
    Time-Slicing=100 & 5 & Baseline MMD & 0.788 & 0.178 & 0.602 & 0.956 \\
    Time-Slicing=100 & 5 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 5 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 5 & Baseline Regression-Fit & 0.327 & 0.218 & 0.144 & 0.568 \\
    Time-Slicing=100 & 5 & Baseline Regression-P & 0.445 & 0.154 & 0.274 & 0.572 \\
    Time-Slicing=100 & 5 & Baseline Wasserstein & 0.005 & 0.008 & 0.001 & 0.014 \\
    Time-Slicing=100 & 5 & MMD CV-AGG & 0.007 & 0.006 & 0.002 & 0.014 \\
    Time-Slicing=100 & 5 & MMD Selection & 0.002 & 0.000 & 0.002 & 0.002 \\ \hline
    
    Time-Slicing=300 & 2 & Baseline MMD & 0.750 & 0.189 & 0.562 & 0.940 \\
    Time-Slicing=300 & 2 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=300 & 2 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=300 & 2 & Baseline Regression-Fit & 0.769 & 0.089 & 0.680 & 0.858 \\
    Time-Slicing=300 & 2 & Baseline Regression-P & 0.862 & 0.053 & 0.822 & 0.922 \\
    Time-Slicing=300 & 2 & Baseline Wasserstein & 0.002 & 0.001 & 0.001 & 0.002 \\
    Time-Slicing=300 & 2 & MMD CV-AGG & 0.005 & 0.005 & 0.002 & 0.010 \\
    Time-Slicing=300 & 2 & MMD Selection & 0.002 & 0.000 & 0.002 & 0.002 \\ \hline
    
    Time-Slicing=500 & 1 & Baseline MMD & 0.871 & 0.145 & 0.704 & 0.964 \\
    Time-Slicing=500 & 1 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=500 & 1 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=500 & 1 & Baseline Regression-Fit & 0.597 & 0.058 & 0.552 & 0.662 \\
    Time-Slicing=500 & 1 & Baseline Regression-P & 0.632 & 0.151 & 0.542 & 0.806 \\
    Time-Slicing=500 & 1 & Baseline Wasserstein & 0.048 & 0.069 & 0.001 & 0.127 \\
    Time-Slicing=500 & 1 & MMD CV-AGG & 0.017 & 0.025 & 0.002 & 0.046 \\
    Time-Slicing=500 & 1 & MMD Selection & 0.002 & 0.000 & 0.002 & 0.002 \\
    \bottomrule
    \end{tabular}    
    \caption{Corresponding information to Fig~\ref{fig:2024-03-12-p-values}. This table shows time buckets where the noise exists. Traceback to \ref{sec:2024-03-12}. \textcolor{blue}{this table will be in an appendix}. \textcolor{red}{Use textbf at the lowest (best) p-value}}
    \label{tab:2024-03-12-p-value-agg}
\end{table}



\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/var_detection_detection/Precision.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/var_detection_detection/Recall.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/var_detection_detection/F.png}
        \caption{Evaluation score of variable detection. Eval. definition is at \protect\hyperlink{2024-03-12-eval-rejection}{here}. Variable detection at the first time bucket where a p-value <= 0.05, see Fig~\ref{fig:2024-03-12-p-values}. Evaluation scores all 0.0 if p-value > 0.05. Traceback to \ref{sec:2024-03-12}.}
        \label{fig:2024-03-12-variable-detection-at-prediction}
    \end{figure*}
\end{multicols}


\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/var_detection_truth/Precision.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/var_detection_truth/Recall.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-standard/var_detection_truth/F.png}
        \caption{
        Evaluation score of variable detection where ground-truth is blue stars in Fig~\ref{fig:2024-03-12-p-values}. 
        Eval. definition is at \protect\hyperlink{2024-03-12-eval-truth}{here}. 
        Evaluation regardless p-value at ground-truth time buckets. 
        Evaluation scores are zero when no variables detected, which is an issue of "Mskernel"; See the technical note~\protect\ref{sec:technical-note-mskernel}. Traceback to \protect Sec.\ref{sec:2024-03-12}. See also \protect\hyperlink{2024-03-12-analysis-self-comment}{my comment}.
        }
        \label{fig:2024-03-12-variable-detection-at-truth}
    \end{figure*}
\end{multicols}


\subsubsection{Log 2024-03-13}
\label{sec:2024-03-13}

\paragraph{Summary}

\begin{figure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/data-visualization/data-0.png}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/data-visualization/data-1.png}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/data-visualization/data-2.png}
    \end{subfigure}
    \caption{
    Synthetic generated time-series in 3 iterations; each column, one data.
    The upper rows are time-series of noised-dimension.
    The blue dashed-lines are time spans where the noise exists.
    The bottom rows are one of time-series without the noise.
    Traceback to \ref{sec:2024-03-13}.
    }
    \label{fig:2024-03-13-data-visualization}
\end{figure}

\paragraph{Result}

Fig~\ref{fig:2024-03-13-p-values}, Fig~\ref{fig:2024-03-13-variable-detection-at-truth}, Fig~\ref{fig:2024-03-13-variable-detection-at-truth}.


\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/p_value_sequence_aggregation/pvals-inverse-noise-100-steps.toml.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/p_value_sequence_aggregation/pvals-inverse-noise-300-steps.toml.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/p_value_sequence_aggregation/pvals-inverse-noise-500-steps.toml.png}
        \caption{
        Aggregated P-values and Time-Buckets. 
        Time-Bucket size $\{100, 300, 500\}$ from the left. 
        3 iterations. 
        Color lines represent the average p-value for variable selection methods. 
        The color region is std values. 
        The red dot line in the vertical axis is at $0.05$ of rejecting $H_0$ hypothesis. 
        The blue stars are the ground-truth time-bucket of noise-starting point. 
        Traceback to \ref{sec:2024-03-13}.}
        \label{fig:2024-03-13-p-values}
    \end{figure*}
\end{multicols}


\begin{table}[ht]
    \centering
    \fontsize{6}{7}\selectfont
    \begin{tabular}{ p{2cm} | p{1cm} | p{2.5cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} }
    \toprule
    $|\mathcal{B}|$ & $\mathcal{B}_i$ & Method & $avg(p)$ & $std(p)$ & $min(p)$ & $max(p)$ \\
    \midrule
    Time-Slicing=100 & 3 & Baseline MMD & 0.293 & 0.207 & 0.082 & 0.496 \\
    Time-Slicing=100 & 3 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 3 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 3 & Baseline Regression-Fit & 0.429 & 0.122 & 0.320 & 0.560 \\
    Time-Slicing=100 & 3 & Baseline Regression-P & 0.244 & 0.196 & 0.032 & 0.420 \\
    Time-Slicing=100 & 3 & Baseline Wasserstein & 0.024 & 0.033 & 0.001 & 0.062 \\
    Time-Slicing=100 & 3 & MMD CV-AGG & 0.023 & 0.023 & 0.002 & 0.048 \\
    Time-Slicing=100 & 3 & MMD Selection & 0.004 & 0.003 & 0.002 & 0.008 \\
    Time-Slicing=100 & 4 & Baseline MMD & 0.607 & 0.274 & 0.322 & 0.868 \\
    Time-Slicing=100 & 4 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 4 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 4 & Baseline Regression-Fit & 0.568 & 0.172 & 0.376 & 0.708 \\
    Time-Slicing=100 & 4 & Baseline Regression-P & 0.457 & 0.125 & 0.318 & 0.558 \\
    Time-Slicing=100 & 4 & Baseline Wasserstein & 0.508 & 0.227 & 0.260 & 0.707 \\
    Time-Slicing=100 & 4 & MMD CV-AGG & 0.760 & 0.151 & 0.672 & 0.934 \\
    Time-Slicing=100 & 4 & MMD Selection & 0.415 & 0.418 & 0.116 & 0.892 \\
    Time-Slicing=100 & 5 & Baseline MMD & 0.545 & 0.219 & 0.318 & 0.754 \\
    Time-Slicing=100 & 5 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 5 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=100 & 5 & Baseline Regression-Fit & 0.417 & 0.217 & 0.258 & 0.664 \\
    Time-Slicing=100 & 5 & Baseline Regression-P & 0.470 & 0.017 & 0.452 & 0.486 \\
    Time-Slicing=100 & 5 & Baseline Wasserstein & 0.001 & 0.000 & 0.001 & 0.001 \\
    Time-Slicing=100 & 5 & MMD CV-AGG & 0.315 & 0.510 & 0.014 & 0.904 \\
    Time-Slicing=100 & 5 & MMD Selection & 0.007 & 0.009 & 0.002 & 0.018 \\ \hline
    
    Time-Slicing=300 & 2 & Baseline MMD & 0.838 & 0.120 & 0.746 & 0.974 \\
    Time-Slicing=300 & 2 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=300 & 2 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=300 & 2 & Baseline Regression-Fit & 0.848 & 0.065 & 0.774 & 0.898 \\
    Time-Slicing=300 & 2 & Baseline Regression-P & 0.782 & 0.074 & 0.716 & 0.862 \\
    Time-Slicing=300 & 2 & Baseline Wasserstein & 0.352 & 0.292 & 0.035 & 0.611 \\
    Time-Slicing=300 & 2 & MMD CV-AGG & 0.351 & 0.361 & 0.018 & 0.734 \\
    Time-Slicing=300 & 2 & MMD Selection & 0.213 & 0.085 & 0.124 & 0.292 \\ \hline
    
    Time-Slicing=500 & 1 & Baseline MMD & 0.654 & 0.203 & 0.454 & 0.860 \\
    Time-Slicing=500 & 1 & Baseline MsKernel Gaussian & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=500 & 1 & Baseline MsKernel IMQ & 1.000 & 0.000 & 1.000 & 1.000 \\
    Time-Slicing=500 & 1 & Baseline Regression-Fit & 0.849 & 0.090 & 0.778 & 0.950 \\
    Time-Slicing=500 & 1 & Baseline Regression-P & 0.753 & 0.034 & 0.726 & 0.792 \\
    Time-Slicing=500 & 1 & Baseline Wasserstein & 0.663 & 0.286 & 0.336 & 0.866 \\
    Time-Slicing=500 & 1 & MMD CV-AGG & 0.765 & 0.172 & 0.610 & 0.950 \\
    Time-Slicing=500 & 1 & MMD Selection & 0.777 & 0.194 & 0.580 & 0.968 \\
    \bottomrule
    \end{tabular}    
    \caption{Corresponding information to Fig~\ref{fig:2024-03-13-p-values}. This table shows time buckets where the noise exists. Traceback to \ref{sec:2024-03-13}. \textcolor{blue}{this table will be in an appendix}. \textcolor{red}{Use textbf at the lowest (best) p-value}}
    \label{tab:2024-03-13-p-value-agg}
\end{table}


\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/var_detection_detection/Precision.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/var_detection_detection/Recall.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/var_detection_detection/F.png}
        \caption{Evaluation score of variable detection. Eval. definition is at \protect\hyperlink{2024-03-12-eval-rejection}{here}. Variable detection at the first time bucket where a p-value <= 0.05, see Fig~\ref{fig:2024-03-13-p-values}. Evaluation scores all 0.0 if p-value > 0.05. Traceback to \ref{sec:2024-03-13}.}
        \label{fig:2024-03-13-variable-detection-at-prediction}
    \end{figure*}
\end{multicols}



\begin{multicols}{3}
    \begin{figure*}[ht!]
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/var_detection_truth/Precision.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/var_detection_truth/Recall.png} \hfill
        \includegraphics[width=.3\textwidth]{images/experiment_records/systhetic_simpler_setting/assessment_run_feat_84/5-dims/noise-inverse/var_detection_truth/F.png}
        \caption{
        Evaluation score of variable detection where ground-truth is blue stars in Fig~\ref{fig:2024-03-13-p-values}. 
        Eval. definition is at \protect\hyperlink{2024-03-12-eval-truth}{here}. 
        Evaluation regardless p-value at ground-truth time buckets. 
        Evaluation scores are zero when no variables detected, which is an issue of "Mskernel"; See the technical note~\protect\ref{sec:technical-note-mskernel}. Traceback to \protect Sec.\ref{sec:2024-03-13}. See also \protect\hyperlink{2024-03-12-analysis-self-comment}{my comment}.
        }
        \label{fig:2024-03-13-variable-detection-at-truth}
    \end{figure*}
\end{multicols}

